Self-Correction Inside the Model: Leveraging Layer Attention to Mitigate Hallucinations in Large Vision Language Models

Although Large Vision-Language Models (LVLMs) have made substantial progress, hallucination, where generated text is not grounded in the visual input, remains a challenge. As LVLMs become stronger, previously reported hallucination patterns, such as linguistic bias and overthinking phenomenon, become far less consistent, making the corresponding mitigation techniques substantially less effective. In this paper, we introduce an Internal self-Correction mechanism utilizing Layer Attention (ICLA) that operates directly on hidden states during generation. Each layer selectively retrieves information from all preceding layers through a diagonal cross-layer attention mechanism, enabling self-refinement without any external correction signals. With introducing and training only 0.2M and 0.1M additional parameters on LLaVA1.5-7B and Qwen2.5-VL-7B, \ours consistently improves visual grounding across multiple hallucination benchmarks, demonstrating its effectiveness for more advanced LVLMs.

==> 1_abstract.tex <==
% \begin{abstract}
% Despite the impressive progress of Large Vision-Language Models (LVLMs), hallucination—where the generated text is not grounded in the visual input—remains a significant challenge. Recent inference-time intervention approaches attempt to address this issue, but they are typically applied in a passive and local manner, inadvertently hindering the flow of shallow visual signals into deeper layers—an essential process for mitigating hallucinations. To address these limitations, we propose CLAM, a decoding-time \textbf{C}ross-\textbf{L}ayer \textbf{A}ttention \textbf{M}echanism that actively and globally retrieves and integrates informative signals from earlier transformer layers. CLAM enables each decoding step to dynamically access relevant historical representations, reinforcing visual grounding without requiring additional inputs. Experiments on various benchmarks demonstrate that CLAM consistently mitigates hallucinations over challenging baselines, demonstrating the effectiveness of our proposed CLAM.
% \end{abstract}


% \begin{abstract}
% Despite the impressive progress achieved by Large Vision-Language Models (LVLMs), hallucination—where the generated text is not grounded in the visual input—remains a significant challenge.
% Existing approaches mitigate this issue either after generation (self-reflection or fine-tuning) or through decoding-time guidance (contrastive decoding), both relying on external correction signals. In this paper, we introduce an \textbf{\underline{I}}nternal self-\textbf{\underline{C}}orrection mechanism utilizing \textbf{\underline{L}}ayer \textbf{\underline{A}}ttention (\textbf{ICLA}) that operates within the model’s hidden states during generation, enabling LVLMs to dynamically retrieve and reconcile information from previous layers to suppress inconsistent representations.
% Without relying on any external correction, our method introduces only 0.2M additional trainable parameters while allowing the model to adaptively integrate prior contextual cues for hallucination mitigation. Experiments across multiple benchmarks demonstrate that our method outperforms several externally guided approaches, highlighting a promising internal pathway for enabling LVLMs to enhance their own reliability without external signals.



% \end{abstract}


\begin{abstract}
Although Large Vision Language Models (LVLMs) have made substantial progress, hallucination, where generated text is not grounded in the visual input, remains a challenge. As LVLMs become stronger, previously reported hallucination patterns, including linguistic bias and the so called “overthinking” phenomenon, become far less consistent, making many existing mitigation techniques substantially less effective.

We introduce an \textbf{\underline{I}}nternal self \textbf{\underline{C}}orrection mechanism with cross \textbf{\underline{L}}ayer \textbf{\underline{A}}ttention (\textbf{ICLA}) that operates directly on hidden states during generation. Each layer selectively retrieves information from all preceding layers through a diagonal cross layer attention mechanism, enabling self refinement without any external correction signals. This design helps the model reconcile inconsistent representations while avoiding cross position interference.

With only 0.2M and 0.1M additional parameters on LLaVA1.5-7B and Qwen2.5-VL-7B, \textbf{ICLA} consistently improves grounding across multiple hallucination benchmarks and achieves state of the art performance on Qwen2.5-VL-7B, demonstrating its effectiveness for modern LVLMs.
\end{abstract}
